SEAN: Image Synthesis with Semantic Region-Adaptive Normalization

We propose semantic region-adaptive normalization (SEAN), a simple but effective building block for Generative Adversarial Networks conditioned on segmentation masks that describe the semantic regions in the desired output image. Using SEAN normalization, we can build a network architecture that can control the style of each semantic region individually, e.g., we can specify one style reference image per region. SEAN is better suited to encode, transfer, and synthesize style than the best previous method in terms of reconstruction quality, variability, and visual quality. We evaluate SEAN on multiple datasets and report better quantitative metrics (e.g. FID, PSNR) than the current state of the art. SEAN also pushes the frontier of interactive image editing. We can interactively edit images by changing segmentation masks or the style for any given region. We can also interpolate styles from two reference images per region.

==> Images/ADEComparison.tex <==
\addtolength{\tabcolsep}{-4.5pt}    
% \setlength{\mywidth}{0.1932\textwidth}
\bgroup
\def\arraystretch{0.5}%  1 is the default. Controls vertical spacing.
\begin{figure*}[]
\begin{tabular} {cc|cc|c}
 Label & Ground Truth & Pix2PixHD~\cite{wang2018pix2pixHD} &  SPADE~\cite{park2019SPADE} & Ours\\
\includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/label/ADE_val_00000146.png} & \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/gt/ADE_val_00000146.jpg} &
\includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/pix2pixhd/ADE_val_00000146.jpg} &   \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/spade/ADE_val_00000146.jpg} &  \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/ours/ADE_val_00000146.png} \\

% \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/label/ADE_val_00000244.png} & \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/gt/ADE_val_00000244.png} &
% \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/pix2pixhd/ADE_val_00000244.png} &   \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/spade/ADE_val_00000244.png} &  \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/ours/ADE_val_00000244.png} \\


% \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/label/ADE_val_00000309.png} & \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/gt/ADE_val_00000309.png} &
% \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/pix2pixhd/ADE_val_00000309.png} &   \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/spade/ADE_val_00000309.png} &  \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/ours/ADE_val_00000309.png} \\

\includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/label/ADE_val_00000532.png} & \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/gt/ADE_val_00000532.jpg} &
\includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/pix2pixhd/ADE_val_00000532.jpg} &   \includegraphics[width=0.1932\textwidth,height=0.80in]{Images/Rec/ADE/spade/ADE_val_00000532.jpg} &  \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/ours/ADE_val_00000532.png} \\

% \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/label/ADE_val_00000967.png} & \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/gt/ADE_val_00000967.png} &
% \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/pix2pixhd/ADE_val_00000967.png} &   \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/spade/ADE_val_00000967.png} &  \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/ours/ADE_val_00000967.png} \\

% \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/label/ADE_val_00001090.png} & \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/gt/ADE_val_00001090.png} &
% \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/pix2pixhd/ADE_val_00001090.png} &   \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/spade/ADE_val_00001090.png} &  \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/ours/ADE_val_00001090.png} \\

% \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/label/ADE_val_00001243.png} & \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/gt/ADE_val_00001243.png} &
% \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/pix2pixhd/ADE_val_00001243.png} &   \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/spade/ADE_val_00001243.png} &  \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/ours/ADE_val_00001243.png} \\


% \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/label/ADE_val_00001517.png} & \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/gt/ADE_val_00001517.png} &
% \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/pix2pixhd/ADE_val_00001517.png} &   \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/spade/ADE_val_00001517.png} &  \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/ours/ADE_val_00001517.png} \\

% \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/label/ADE_val_00000090.png} & \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/gt/ADE_val_00000090.png} &
% \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/pix2pixhd/ADE_val_00000090.png} &   \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/spade/ADE_val_00000090.png} &  \includegraphics[width=0.1932\textwidth,height=0.96in]{Images/Rec/ADE/ours/ADE_val_00000090.png} \\

\end{tabular}
\vspace{-2mm}
	\caption{Visual  comparison  of  semantic  image  synthesis  results  on  the ADE20K. We compare Pix2PixHD, SPADE, and our method.}
	\label{fig:ADE20K results}	
\vspace{-3mm}	
 \end{figure*}
 \egroup
 \addtolength{\tabcolsep}{4.5pt}

==> Images/CelebAComparison.tex <==
\addtolength{\tabcolsep}{-4.5pt}    
% \setlength{\mywidth}{0.1932\textwidth}
\bgroup
\def\arraystretch{0.5}%  1 is the default. Controls vertical spacing.
\begin{figure*}[]
\begin{tabular} {cc|cc|c}
 Label & Ground Truth & Pix2PixHD~\cite{wang2018pix2pixHD} &  SPADE~\cite{park2019SPADE} & Ours\\
% \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/label/28016.png} & \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/gt/28016.png} &
% \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/pix2pixhd/28016.png} &   \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/spade/28016.png} &  \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/ours/28016.png} \\

\includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/label/28360.png} & \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/gt/28360.jpg} &
\includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/pix2pixhd/28360.jpg}&jpg
\includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/spade/28360.jpg} &  \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/ours/28360.png} \\

% \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/label/28054.png} & \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/gt/28054.png} &
% \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/pix2pixhd/28054.png}&
% \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/spade/28054.png} &  \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/ours/28054.png} \\

\includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/label/28181.png} & \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/gt/28181.jpg} &
\includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/pix2pixhd/28181.jpg}&
\includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/spade/28181.jpg} &  \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/ours/28181.png} \\

% \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/label/28434.png} & \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/gt/28434.png} &
% \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/pix2pixhd/28434.png}&
% \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/spade/28434.png} &  \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/ours/28434.png} \\

% \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/label/28059.png} & \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/gt/28059.png} &
% \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/pix2pixhd/28059.png}&
% \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/spade/28059.png} &  \includegraphics[width=0.1932\textwidth]{Images/Rec/Faces/ours/28059.png} \\


\end{tabular}
\vspace{-2mm}
	\caption{Visual  comparison  of  semantic  image  synthesis  results  on  the  CelebAMask-HQ dataset. We compare Pix2PixHD, SPADE, and our method.}
	\label{fig:CelebAMask-HQ results}	
\vspace{-3mm}	
 \end{figure*}
 \egroup
 \addtolength{\tabcolsep}{4.5pt}

==> Images/CityScapeComparison.tex <==
jpg\addtolength{\tabcolsep}{-4.5pt}    
% \setlength{\mywidth}{0.1932\textwidth}
\bgroup
\def\arraystretch{0.5}%  1 is the default. Controls vertical spacing.
\begin{figure*}[]
\begin{tabular} {cc|cc|c}
 Label & Ground Truth & Pix2PixHD~\cite{wang2018pix2pixHD} &  SPADE~\cite{park2019SPADE} & Ours\\
\includegraphics[width=0.1932\textwidth]{Images/Rec/CityScape/label/munster_000017_000019_leftImg8bit.png} & \includegraphics[width=0.1932\textwidth]{Images/Rec/CityScape/gt/munster_000017_000019_leftImg8bit.jpg} &
\includegraphics[width=0.1932\textwidth]{Images/Rec/CityScape/pix2pixhd/munster_000017_000019_leftImg8bit.jpg} &   \includegraphics[width=0.1932\textwidth]{Images/Rec/CityScape/spade/munster_000017_000019_leftImg8bit.jpg} &  \includegraphics[width=0.1932\textwidth]{Images/Rec/CityScape/ours/munster_000017_000019_leftImg8bit.png} \\
 
% \includegraphics[width=0.1932\textwidth]{Images/Rec/CityScape/label/frankfurt_000000_022254_leftImg8bit.png} & \includegraphics[width=0.1932\textwidth]{Images/Rec/CityScape/gt/frankfurt_000000_022254_leftImg8bit.png} &
% \includegraphics[width=0.1932\textwidth]{Images/Rec/CityScape/pix2pixhd/frankfurt_000000_022254_leftImg8bit.png} &   \includegraphics[width=0.1932\textwidth]{Images/Rec/CityScape/spade/frankfurt_000000_022254_leftImg8bit.png} &  \includegraphics[width=0.1932\textwidth]{Images/Rec/CityScape/ours/frankfurt_000000_022254_leftImg8bit.png} \\

\includegraphics[width=0.1932\textwidth]{Images/Rec/CityScape/label/frankfurt_000001_044787_leftImg8bit.png} & \includegraphics[width=0.1932\textwidth]{Images/Rec/CityScape/gt/frankfurt_000001_044787_leftImg8bit.jpg} &
\includegraphics[width=0.1932\textwidth]{Images/Rec/CityScape/pix2pixhd/frankfurt_000001_044787_leftImg8bit.jpg} &   \includegraphics[width=0.1932\textwidth]{Images/Rec/CityScape/spade/frankfurt_000001_044787_leftImg8bit.jpg} &  \includegraphics[width=0.1932\textwidth]{Images/Rec/CityScape/ours/frankfurt_000001_044787_leftImg8bit.png} \\


\end{tabular}
\vspace{-2mm}
	\caption{Visual  comparison  of  semantic  image  synthesis  results  on  the  CityScapes dataset. We compare Pix2PixHD, SPADE, and our method.}
	\label{fig:CityScape results}	
\vspace{-3mm}	
 \end{figure*}
 \egroup
 \addtolength{\tabcolsep}{4.5pt}

==> Images/FACADESComparison.tex <==
% \addtolength{\tabcolsep}{-4.5pt}    
% % \setlength{\mywidth}{0.1932\textwidth}
% \bgroup
% \def\arraystretch{0.5}%  1 is the default. Controls vertical spacing.
% \begin{figure*}[]
% \begin{tabular} {cc|cc|c}
%  Label & Ground Truth & Pix2PixHD~\cite{wang2018pix2pixHD} &  SPADE~\cite{park2019SPADE} & Ours\\
% \includegraphics[width=0.1932\textwidth]{Images/Rec/FACADES/label/Austria_Vienna_relation2188125_Fid2009_MzrGCs1EpkA-bVVhcmNnCg.png} & \includegraphics[width=0.1932\textwidth]{Images/Rec/FACADES/gt/Austria_Vienna_relation2188125_Fid2009_MzrGCs1EpkA-bVVhcmNnCg.png} &
% \includegraphics[width=0.1932\textwidth]{Images/Rec/FACADES/pix2pixhd/Austria_Vienna_relation2188125_Fid2009_MzrGCs1EpkA-bVVhcmNnCg.png} &   \includegraphics[width=0.1932\textwidth]{Images/Rec/FACADES/spade/Austria_Vienna_relation2188125_Fid2009_MzrGCs1EpkA-bVVhcmNnCg.png} &  \includegraphics[width=0.1932\textwidth]{Images/Rec/FACADES/ours/Austria_Vienna_relation2188125_Fid2009_MzrGCs1EpkA-bVVhcmNnCg.png} \\

% \includegraphics[width=0.1932\textwidth]{Images/Rec/FACADES/label/Austria_Vienna_way175776886_Fid1698_QhErsGwv-5YJ9ZlTvv1I8w.png} & \includegraphics[width=0.1932\textwidth]{Images/Rec/FACADES/gt/Austria_Vienna_way175776886_Fid1698_QhErsGwv-5YJ9ZlTvv1I8w.png} &
% \includegraphics[width=0.1932\textwidth]{Images/Rec/FACADES/pix2pixhd/Austria_Vienna_way175776886_Fid1698_QhErsGwv-5YJ9ZlTvv1I8w.png}&
% \includegraphics[width=0.1932\textwidth]{Images/Rec/FACADES/spade/Austria_Vienna_way175776886_Fid1698_QhErsGwv-5YJ9ZlTvv1I8w.png} &  \includegraphics[width=0.1932\textwidth]{Images/Rec/FACADES/ours/Austria_Vienna_way175776886_Fid1698_QhErsGwv-5YJ9ZlTvv1I8w.png} \\


% \end{tabular}
% \vspace{-2mm}
% 	\caption{Visual  comparison  of  semantic  image  synthesis  results  on  the \Facades  dataset. Pix2PixHD uses the default feature encoder and SPADE uses the default style image encoder.}
% 	\label{fig:FACADES results}		
% \vspace{-3mm}	
%  \end{figure*}
%  \egroup
%  \addtolength{\tabcolsep}{4.5pt}

\addtolength{\tabcolsep}{-4.5pt}    
% \setlength{\mywidth}{0.1932\textwidth}
\bgroup
\def\arraystretch{0.5}%  1 is the default. Controls vertical spacing.
\begin{figure}[]
\small
\begin{tabular} {cc|cc|c}
 Label & GT & Pix2PixHD &  SPADE & Ours\\
% \includegraphics[width=0.09\textwidth]{Images/Rec/FACADES/label/Austria_Vienna_relation2188125_Fid2009_MzrGCs1EpkA-bVVhcmNnCg.png} & \includegraphics[width=0.09\textwidth]{Images/Rec/FACADES/gt/Austria_Vienna_relation2188125_Fid2009_MzrGCs1EpkA-bVVhcmNnCg.png} &
% \includegraphics[width=0.09\textwidth]{Images/Rec/FACADES/pix2pixhd/Austria_Vienna_relation2188125_Fid2009_MzrGCs1EpkA-bVVhcmNnCg.png} &   \includegraphics[width=0.09\textwidth]{Images/Rec/FACADES/spade/Austria_Vienna_relation2188125_Fid2009_MzrGCs1EpkA-bVVhcmNnCg.png} &  \includegraphics[width=0.09\textwidth]{Images/Rec/FACADES/ours/Austria_Vienna_relation2188125_Fid2009_MzrGCs1EpkA-bVVhcmNnCg.png} \\

\includegraphics[width=0.09\textwidth]{Images/Rec/FACADES/label/Austria_Vienna_way175776886_Fid1698_QhErsGwv-5YJ9ZlTvv1I8w.png} & \includegraphics[width=0.09\textwidth]{Images/Rec/FACADES/gt/Austria_Vienna_way175776886_Fid1698_QhErsGwv-5YJ9ZlTvv1I8w.jpg} &
\includegraphics[width=0.09\textwidth]{Images/Rec/FACADES/pix2pixhd/Austria_Vienna_way175776886_Fid1698_QhErsGwv-5YJ9ZlTvv1I8w.jpg}&
\includegraphics[width=0.09\textwidth]{Images/Rec/FACADES/spade/Austria_Vienna_way175776886_Fid1698_QhErsGwv-5YJ9ZlTvv1I8w.jpg} &  \includegraphics[width=0.09\textwidth]{Images/Rec/FACADES/ours/Austria_Vienna_way175776886_Fid1698_QhErsGwv-5YJ9ZlTvv1I8w.png} \\


\end{tabular}
\vspace{-2mm}
	\caption{Visual  comparison  of  semantic  image  synthesis  results  on  the \Facades dataset. We compare Pix2PixHD, SPADE, and our method.}
	\label{fig:FACADES results}		
\vspace{-3mm}	
 \end{figure}
 \egroup
 \addtolength{\tabcolsep}{4.5pt}
